Quantifying Process Quality: The Role of Effective Organizational Learning in Software Evolution

Real-world software applications must constantly evolve to remain relevant. This evolution occurs when developing new applications or adapting existing ones to meet new requirements, make corrections, or incorporate future functionality. Traditional methods of software quality control involve software quality models and continuous code inspection tools. These measures focus on directly assessing the quality of the software. However, there is a strong correlation and causation between the quality of the development process and the resulting software product. Therefore, improving the development process indirectly improves the software product, too. To achieve this, effective learning from past processes is necessary, often embraced through post mortem organizational learning. While qualitative evaluation of large artifacts is common, smaller quantitative changes captured by application lifecycle management are often overlooked. In addition to software metrics, these smaller changes can reveal complex phenomena related to project culture and management. Leveraging these changes can help detect and address such complex issues. Software evolution was previously measured by the size of changes, but the lack of consensus on a reliable and versatile quantification method prevents its use as a dependable metric. Different size classifications fail to reliably describe the nature of evolution. While application lifecycle management data is rich, identifying which artifacts can model detrimental managerial practices remains uncertain. Approaches such as simulation modeling, discrete events simulation, or Bayesian networks have only limited ability to exploit continuous-time process models of such phenomena. Even worse, the accessibility and mechanistic insight into such gray- or black-box models are typically very low. To address these challenges, we suggest leveraging objectively [...]

==> chapters/01_Abstract.tex <==
\begin{abstract}
{\small
% Introduction, background
Real-world software applications need to evolve continuously or else become increasingly useless.
Software evolution happens during the development of new applications, or when an existing application is adapted to new requirements, receives corrections, or is changed to accommodate future functionality.
Software quality models and continuous code inspection tools are typical measures for direct software quality control in that situation.
However, not only do we find a significant positive correlation between the quality of the development process and the manufactured product, but also strong causation.
Improving the process, therefore, constitutes another valid, yet indirect measure to improving the product.
In turn, this requires that we can learn effectively from past processes.
Indeed, this is frequently embraced in post mortem organizational learning.
Using mostly unstructured artifacts that are typically produced during the development, experts engage in qualitative evaluation of past projects.
However, beyond large artifacts, the application lifecycle management that governs software processes typically captures a considerable number of smaller, mostly quantitative changes.
While such small changes were previously leveraged for fault prediction and -prevention, they have not yet been used to detect complex phenomena that manifest not only in software metrics but predominantly in project culture and management.


% Problem?
% Method, how did we try to solve the problem?
% Results/Analysis, what was the outcome?
% Discussion, what do the results mean?
Software evolution was previously captured by the size of the changes made.
However, the lack of a consensus on what constitutes a versatile and robust quantification of the size currently prohibits its usage as a dependable software metric.
Different notions of size were also previously used to capture the nature of each change.
However, these classifications cannot describe the nature of evolution with sufficient reliability.
While application lifecycle management data is typically rich, we do not currently know which artifacts can be leveraged to model managerial anti-patterns, which are malpractices with adverse effects on process quality.
Approaches such as simulation modeling, discrete events simulation, or Bayesian networks have only limited ability to exploit continuous-time process models of such phenomena.
Even worse, the accessibility and mechanistic insight into such gray- or black-box models are typically very low.
%
We suggest that a synthesis of objectively captured digital artifacts from application lifecycle management, together with qualitative analysis can be exploited for efficient organizational learning.
We first propose a new, language-independent metric that can robustly capture the size of changes.
Then, these new size-based measurements are used to considerably boost the classification accuracy of the nature of these changes.
We explore, visualize, and suggest maintenance activities as derived from the classified changes and can reliably predict the presence and severity of malpractice, even from ``little data''.
Lastly, we make parts of the automatic quantitative analysis accessible and allow it to partially replace qualitative expert-based analysis.





}
\bigskip
\vfill
\noindent
\textbf{Keywords:}
Software Size, Software Metrics, Commit Classification, Maintenance Activities, Software Quality, Process Quality, Project Management, Organizational Learning, Machine Learning, Visualization, Optimization

\end{abstract}
\cleardoublepage

